Significance-based community detection in weighted networks

Community detection is the process of grouping strongly connected nodes in a network. Many community detection methods for un-weighted networks have a theoretical basis in a null model. Communities discovered by these methods therefore have interpretations in terms of statistical signficance. In this paper, we introduce a null for weighted networks called the continuous configuration model. We use the model both as a tool for community detection and for simulating weighted networks with null nodes. First, we propose a community extraction algorithm for weighted networks which incorporates iterative hypothesis testing under the null. We prove a central limit theorem for edge-weight sums and asymptotic consistency of the algorithm under a weighted stochastic block model. We then incorporate the algorithm in a community detection method called CCME. To benchmark the method, we provide a simulation framework incorporating the null to plant "background" nodes in weighted networks with communities. We show that the empirical performance of CCME on these simulations is competitive with existing methods, particularly when overlapping communities and background nodes are present. To further validate the method, we present two real-world networks with potential background nodes and analyze them with CCME, yielding results that reveal macro-features of the corresponding systems.

==> section_files/bw_Sec2_Notation.tex <==
\section{Notation and terminology}\label{Notation}

We will denote an undirected weighted network on $n$ nodes by a triple $\mathcal{G}:= (N,E,w)$, where $N := \{1,\ldots,n\}$ is the node set, $E$ is the edge set, consisting of all unordered
node-pairs $\{u,v\}$ for which there is an edge between $u$ and $v$, and $w: N \times N \mapsto [0,\infty)$ 
is a symmetric function that assigns a non-negative weight to each pair of nodes with $w(u,v) = 0$ 
if (and only if) $\{u,v\} \notin E$. The degree of a node $u$ is defined by
$d(u) := \sum_{v \in N} \IND(\{u,v\}\in E)$, and we denote the vector of node degrees by ${\bf d} = (d(1),\ldots,d(n))$.
In an analogous fashion, we define the {\it strength} of a node by
$s(u) := \sum_{v \in N} w(u,v)$, and the strength vector of the network by ${\bf s} = (s(1),\ldots,s(n))$.
The total degree and strength of $\mathcal{G}$ are given by $d_T := \sum_{v \in N} d(v)$ and 
$s_T := \sum_{v \in N} s(v)$, respectively. Given a vector $\vx$ of dimension $n$, we define for any indices $u,v\in N$ the ratio
\begin{equation}\label{ratio}
r_{uv}(\vx) := \frac{x(u)x(v)}{\sum_ux(u)}
\end{equation}
Finally, define $\ruvdag := \min(1,r_{uv}(\vx))$ and $f_{uv}(\vx,\vy) := r_{uv}(\vy)/\ruvdag(\vx)$.


\begin{comment}
For $u \in N$ let 
$\mathcal{C}(u) = \{ C_i : u \in C_i \}$ and
$k(u) = \{ i : u \in C_i \}$ be the elements of $\mathcal{C}$ that contain $u$, 
and the indices of these elements, respectively.

\textbf{Remark.} Our restriction of the range of $w$ to $[0,\infty)$ does not sacrifice much generality. 
In many cases, if the edges of a network have negative weights, one may transform them 
to non-negative weights in a way that preserves relevant community structure. 
\end{comment}


==> section_files/bw_Sec4_2_Consistency.tex <==
\section{Consistency}\label{consistency}

In this section, we evaluate the consistency of the CCME update procedure under a weighted stochastic block model (WSBM). This model closely resembles the continuous configuration model, but has extra parameters to incorporate community structure. The model is similar to that presented in \cite{aicher2014learning}, but is generalized to include node-specific weight parameters.

For fixed $K > 0$, we define a $K$-block WSBM on $n > 1$ nodes as follows. Let $\vc_n$ be the community assignment vector with $c_n(u)\in[K]$ giving the community of $u$. Define $\cC_{i,n}:=\{u:c_n(u) = i\}$ and $\pi_{i,n} := n^{-1}|\cC_i|$. Let $\mM$ and $\mP$ be $K\times K$ matrices with non-negative entries encoding baseline inter-community edge probabilities and inter-community edge weight expectations (respectively). Let $\{\rho_n\}_{n>1}$ be a sequence bounded in the interval $[0,1]$ such that either $\rho_n\equiv1$ or $\rho_n\rightarrow0$. This parameter represents the edge-sparsity of the network. Let $\phi_n$ and $\psi_n$ be arbitrary $n$-vectors with positive entries. Finally, let $\cP$ be an arbitrary probability distribution on the positive real line with mean 1 and variance $\sigma^2>0$. The $K$-WSBM is then specified as follows:
\begin{enumerate}
\item Generate edge $\{u,v\}$ with probability $\mathbb{P}(\{u,v\}\in E) = \rho_nr_{uv}(\phi_n)\mP[c_n(u), c_n(v)]$, independently across node pairs $\{u,v\}$, prohibiting self-loops.
\item{For each edge $\{u,v\}\in E$, generate an independent random variable $\xi(u,v)$ according to $\cP$. Determine edge weight $W(u,v)$ by:
\[
W(u,v) = \begin{cases}
0&\text{if }\{u,v\}\notin E\\
\ffun{\psi_n}{\phi_n}\mM[c_n(u), c_n(v)]\xi(u,v)&\text{if }\{u,v\}\in E
\end{cases}
\]
}
\end{enumerate}
For the above generative model to be well-defined, we require three assumptions. First, we must have $\rho_n\cdot\max(\mP)\cdot\max_{uv}\{r_{uv}(\phi_n)\}\leq1$. Second, for identifiability, we assume the vector-wise means $\bar \phi$ and $\bar\psi$ are equal to $n$. Third (also for identifiability) we assume that the term $\rho_n\mP[c_n(u), c_n(v)]$ may be replaced by $\mP_n[c_n(u),c_n(v)]$ where $\mP_n := \rho_n\mP$.

\subsubsection{Consistency theorem} In the CCME consistency theorem, we make the following basic assumptions on the parameters of each $n$-indexed WSBM that are common among other consistency analyses of community detection algorithms (e.g.\  \cite{zhao2012consistency}):

%%%%%%%%%
%%% Assumptions
%%%%%%%%%

\begin{assumption}\label{community-size-assumption} There exists $\tau>0$ such that $\min_i\pi_{i,n}\geq\tau$ for all $n> 1$.
\end{assumption}
\begin{assumption}\label{bounded-parameter-assumption} There exist constants $m_+>m_->0$ such that, for all $n>1$, the entries of $\phi_n$, $\psi_n$, $\mP$, and $\mM$ are bounded in the interval $[m_-,m_+]$.
\end{assumption}
We also make the following assumption which is necessitated by our particular framework:
\begin{assumption}\label{bounded-weight-assumption} $\mathcal{P}$ has support bounded by $\nu<\infty$ independent of $n$.
\end{assumption}
Assumption \ref{bounded-weight-assumption} allows the use of Bernstein's inequality throughout the proof. This assumption may be relaxed if there are constraints on the moments of $\mathcal{P}$ allowing the use of a similar inequality.

We adapt notation used throughout Sections \ref{Model}-\ref{Method}, as follows. Similar to Equation \eqref{Model:expv1}, for each $n>1$ and any node $u\in[n]$, let $S_n(u)$ be the (random) strength of $u$ from the $n$-th random network $\Net_n$ and define $\tilde s_n(u) := \expv \{S_n(u)\}$. Define $D_n(u)$ and $\tilde d_n(u)$ analogously for $u$'s degree. Let $S_n(u:B)$ be the CCME test-statistic from $\Net_n$, as in the set-up of Theorem \ref{thm:CLT}. With the functions $\mu$ and $\sigma$ from

Some further notation is needed. For nodes $u,v\in[n]$ and two $n$-vectors $\vx$,$\vy$ with positive entries, define
\begin{equation}\label{vuv}
\tilde v_{uv}(\vy,\vx) := \expv\left\{\left(W(u,v) - f_{uv}(\vy,\vx)\right)^2\big|\{u,v\}\in E\right\}
\end{equation}
Define the population variance estimator as follows:
\begin{equation}\label{pop-var}
\tilde \theta(\vy,\vx) := \frac{\sum_{uv\in E}\tilde v_{uv}(\vy,\vx)}{\sum_{uv\in E}f_{uv}(\vy,\vx)^2}
\end{equation}


%%%%%%%%%
%%% Theorem
%%%%%%%%%

\begin{theorem}\label{initial-to-community}
Fix $K>1$. For each $n > 1$, let $\cG_n$ be a random network generated by a $K$-WSBM with $n>1$ nodes and parameters satisfying Assumptions \ref{community-size-assumption} - \ref{bounded-weight-assumption}. Suppose further that $\win\pin>\wout\pout$, and that for any fixed $\kappa>0$, $\frac{(\log n)^\kappa}{\rho_nn}\rightarrow0$ as $n\rightarrow\infty$. Fix $i\in[K]$. Let $\{B_n\}_{n>1}$ be a sequence of node sets satisfying the following: there exist constants $q\in(0,1)$ and $\Delta>0$ such that for all $n>1$, $|B_n|\geq qn$, and
\begin{equation}\label{favors}
\frac{\expv S(u:B_n) - \mfun{u}{B_n}{\tilde\vs}}{\sfun{u}{B_n}{\tilde\vs}{\tilde\vd}{\theta}}\begin{cases}
\geq \Delta\sqrt{\rho_n n},&u\in\cC_i\\
\leq -\Delta\sqrt{\rho_n n},&u\notin\cC_i
\end{cases}
\end{equation}
Then
\[
\mathbb{P}\big(U_\alpha(B_n, \cG_n) = \cC_i\big)\rightarrow1\text{ as }n\rightarrow\infty
\]
\end{theorem}

In essence, Theorem \ref{initial-to-community} says that recovery of community $\cC_i$ is from a particular set $B_n$ is asymptotically guaranteed with high probability, providing the limiting value of {\color{red}$Z_n(u:B_n)$} ``favors" nodes from $\cC_i$. By ``favors" we mean explicitly the relation given by the inequalities in \eqref{favors}: $\tilde z_n(u:B_n)$ must be positive for $u\in\cC_i$ and negative for $u\notin\cC_i$.

It remains then to consider what sequences $\{B_n\}_{n>1}$ are ``favorable" with respect to a certain community sequence $\{C_{i,n}\}_{n>1}$. lead to recovery of a particular community $\cC_i$. We should expect, loosely speaking, that each $B_n$ must be ``dominated" by nodes from $\cC_i$ at some minimum level determined by $\mP$ and $\mM$.



==> section_files/bw_Sec4_Method2.tex <==
\section{The CCME method and algorithm}\label{Method}

In this section we describe the components of the CCME method. 
Given an observed weighted network $\Net$, CCME begins by identifying a collection of initializing node sets. 
Proceeding sequentially through this collection, the method iteratively updates each set through 
node-wise hypothesis tests. Thus each initial set is the beginning of an iterative chain of node sets. 
If the chain converges to a non-empty node set, the limiting set is added to a collection of ``found" 
communities from which the output of the method is derived. 
We give a precise description of the procedure in the following sections.



\subsection{Initialization}\label{Method:initialization}

%The CCME method relies on initial node sets that are each somewhat dominated, proportionally, by a true community. 
%We introduce a procedure to this end based on statistics informed by continuous configuration model. 

Given an observed weighted network $\Net$, the CCME method begins by identifying a collection of 
initial node sets, one for each node of the network. 
For a fixed node $u \in [n]$, we measure the preference of node $v$ for $u$ by
\[
z(v) := \max\left\{\dfrac{w(u,v) - s_{uv}/d_{uv}}{\sqrt{\theta}s_{uv}/d_{uv}},\;0\right\}
\]
where $\theta$ is the variance parameter of the continuous configuration model derived from the observed network.
The measure $z(v)$ acts like a truncated $z$-type statistic, quantifying the extremity of the weight $w(u,v)$. 
The initial node set corresponding to $u$, denoted by $B_0(u)$, is formed by sampling $d(u)$ nodes with 
replacement from $[n]$ with probability proportional to $z(v)$. 
%ABN: Some justification for turning z-like stats into probabilities??
Note that if $u$ is part of a community, then the measure $z(v)$ for nodes $v$ in the community 
will be larger (on average) than other nodes.  We denote the set of initial sets by $\mathcal{B}_0 := \{ B_0(u) : u \in [n] \}$.


\subsection{Set update}
\label{Method:update}
The CCME method proceeds by performing iterative set updates on each initial node set. 
The update of a node set $B$ adds or retains nodes preferentially connected to $B$, 
and ignores or expels nodes that are not preferentially connected to $B$. 
This procedure is based on the statistic
\begin{equation}\label{eq:test_stat}
s(u:B) := \sum_{v \in B} w(u,v),
\end{equation}
which measures the strength of the connection between $u$ and $B$.
When the (observed) value of $s(u:B)$ is larger than its expectation under the 
continuous configuration model, there is evidence to support a connection 
between $u$ and $B$ resulting from some form of community structure in the network. 
To assess the significance of $s(u:B)$ (the strength of evidence), we compute the p-value
\begin{equation}\label{eq:pvalue}
p(u : B) := \prob\left\{ \hat{s}(u:B) > s(u:B) \right\}.
\end{equation}%\label{eq:hypotheses}
where $\hat{s}(u:B)$ denotes the (random) value of $s(u:B)$ under the continuous 
configuration model, and $\prob()$ denotes the measure on $n$-node networks induced
by the model.

%Note that under the null specification described in section \ref{Model:properties}, the expectation of $\hat{s}(u:B)$ under the continuous configuration model is $s(u)s(B)/s_T$, where $s(B) := \sum_{v\in B}s(v)$. Thus, the p-value in \eqref{eq:pvalue} can be thought of as associated with the following test:
%\begin{equation}\label{eq:hypotheses}
%H_0:\;\expv\left[\tilde{s}(u:B)\right]  = \frac{s(u)s(B)}{s_T}
%\;\;\;\text{vs.}\;\;\;
%H_1:\;\expv\left[\tilde{s}(u:B)\right]  > \frac{s(u)s(B)}{s_T}
%\end{equation}
%where $\tilde{s}(u:B)$ is a random with respect to the ``true" systematic behavior of the network.

%ABN: A bit more detail here, as this step is important.
To update $B$, we calculate $p(u:B)$ for every node, and form the updated set from the nodes corresponding to the p-values that are significant after adjusting for multiple tests. The multiple-testing adjustment we use is the false discovery rate (FDR) control procedure of 
Benjamini and Hochberg \cite{benjamini1995controlling}. Given a set of p-values ${\bf p} := \{p_i\}_{i \leq n}$ corresponding 
to $n$ hypothesis tests and a target FDR $\alpha\in(0, 1)$, each p-value $p_i \in {\bf p}$ is associated with an 
adjusted p-value $p_i^\ast := n \, p_i \, / \, j(i)$ where $j(i)$ is the rank of $p_i$ in ${\bf p}$.  The Benjamini-Hochberg 
procedure rejects hypotheses $i$ for which $p_i$ is less than or equal to the threshold 
$\tau_{\text{BH}} := \max\{p_i\;:\;p_i^\ast\leq\alpha\}$.

In subsequent sections, we denote the entire set-update procedure 
(from p-value computation to FDR control) as the map 
$\Salph: \mathbbm{2}^{[n]} \mapsto \mathbbm{2}^{[n]}$, where $\mathbbm{2}^{[n]}$ is all subsets of $[n]$, $\alpha$ is the specified FDR, and $\Net$ is the observed network. 
The value of $\alpha$ is thus a parameter of CCME which must be set by protocol, though we recommend the setting $\alpha = 0.05$ (used throuought the analyses in Sections \ref{Simulations} and \ref{Data}).

%We note that for distinct nodes $u$ and $v$, the random variables $\hat s(u:B)$ and $\hat s(v:B)$ under the continuous configuration model are correlated only when $u,v\in B$. This correlation is positive through $u$ and $v$'s shared edge. As the Benjamini-Hochberg procedure is valid for correlated tests, this fact justifies its use.
%For maximal clarity, we give the pseudo-code for the set-update procedure in the Appendix.


\subsection{Asymptotic Normality of $\hat s(u:B)$}\label{Method:CLT}

In most cases the distribution of the variable $\hat{s}(u:B)$ appearing in \eqref{eq:pvalue} 
is not analytically intractable, and therefore the p-value $p(u:B)$ cannot be calculated exactly. 
In this section, we state a central limit theorem that yields a closed-form approximation for  
$p(u:B)$ that can be computed quickly.

\subsubsection{Setting and theorem}
Suppose we are given a sequence of model parameters 
$\{({\bf d}_n, {\bf s}_n, \theta_n, \mathcal{P}_n)\}_{n\geq1}$. For each $n$, a random network 
$\hat \Net_n$ is generated according to the continuous configuration model with parameters 
(${\bf d}_n, {\bf s}_n, \theta_n, \mathcal{P}_n$), as defined in Section \ref{Model:statement}. 
We assume $d_n(u)\geq1$ for all $u\in[n]$ and $d_{uv, n}\leq 1$
(defined in Section \ref{Model:statement}) for all $u,v\in[n]$. 
We consider the asymptotic behavior of $\hat{s}(u:B)$ in this setting
for nodes $u$ and sets $B$ from $\hat{\Net}_n$ as $n\rightarrow\infty$.

Our main result requires certain conditions on the parameter sequence. We will say that a sequence of 
real numbers $\{a_n\}_{n \geq1}$ is bounded away from zero and infinity if 
\[
0 < \underset{n \rightarrow \infty}{\liminf} \; a_n
\;\text{ and }\;
\sup_{n \geq 1} \; a_n < \infty
\]
and that a triangular array $\{ a_n(u) \}_{n \geq1, u \in [n]}$ is \emph{uniformly} bounded away from zero and infinity if
\[
0 < \underset{n\rightarrow\infty}{\liminf} \; \min_{u\in[n]}a_n(u)
\;\text{ and }\;
\sup_{n \geq 1} \; \max_{u \in [n]} a_n(u) < \infty.
\]
%ABN: We might just say bounded away from zero and infinity, with the understanding that the former is ``eventually''
For each $n \geq 1$ let $\lambda_n$ denote the average entry of ${\bf d}_n$, which is the average 
expected degree of $\hat{\Net}_n$.  For each $r \geq 0$ let 
$L_{n, r} := n^{-1} \sum_{u \in [n]} (d_n(u)/\lambda_n)^r$ be the normalized 
$r^{\text{th}}$-moment of ${\bf d}_n$.  Note that $L_{n, 1} = 1$.
We impose the following regularity conditions on the parameters of the networks $\hat \Net_n$.

\noindent
\begin{assumption}\label{assumption:power}
There exists $\beta > 0$ such that the sequence 
\[
\left\{\frac{s_n(u)}{d_n(u)^{1+\beta}}\right\}_{n\geq1, u\in[n]}
\]
is uniformly bounded away from zero and infinity. 
\end{assumption}

\noindent
\begin{assumption}\label{assumption:moment}
There exists $\eps > 0$ such that, with $\beta$ as in Assumption \ref{assumption:power}, both
\[
\{L_{n, 4\beta + 2}\}_{n\geq1} \text{ and } \{L_{n, 4\beta + 2 + \eps}\}_{n\geq1}
\]
are bounded away from zero and infinity.
\end{assumption}

\begin{assumption}\label{assumption:distribution}
The sequence $\{\theta_n\}_{n \geq1}$ is bounded away from zero and infinity, 
and $\{\mathcal{P}_n\}_{n\geq1}$ satisfies
\[
\sup_n\left\{\underset{u,v\in[n]}{\max}\expv\left(\hat\xi_{uv,n}^3\right)\right\}<\infty
\]
\end{assumption}

%These parameter conditions have a trade-off relationship. The value of $\beta$ imposes regularity, via the power-law condition, on the relationship between the degrees and strengths; $\beta =0$ corresponds to the regime where $O(s_n(u)) = O(d_n(u))$ for all $u$. As $\beta$ increases, we require the stability of increasingly higher moments for the normalized degree sequences, via the moment condition. 

Assumption \ref{assumption:power} reflects a frequently observed relationship between strengths and degrees 
in real networks (\cite{barrat04, clauset09}).  Assumption \ref{assumption:moment} is needed to control
the extremal behavior of the degree distribution. It excludes, for instance, cases in which there are 
a few nodes with degree close to $n$ and the degree of the remaining nodes are bounded as $n$ increases.  We note that the condition becomes more stringent as $\beta$ increases, since as $\beta$ increases the strength-degree power law becomes more severe. Assumption \ref{assumption:distribution} ensures boundedness of the second and third moments of the 
distributions in $\{\mathcal{P}_n\}_{n\geq1}$.

%Hub nodes are common in real networks (\cite{mislove2007measurement}, \cite{ahn2007analysis}, \cite{ebel2002scale}, \cite{bryan1999hub}, \cite{csanyi04}, \cite{barabasi99}) and in many simulation frameworks used to benchmark community detection methods. Though the moment condition allows for many types of degree distributions observed in these sources, surely we can not expect it to allow for all types. For some networks with pathological degree sequences, algorithms other than CCME may be required to detect community structure.

%The conditions are also interpretable with respect to existing characterizations of real data. Relationships between strengths and degrees of the form expressed in the power-law condition are commonly seen in real weighted networks \cite{barrat04}, \cite{clauset09}. The moment condition amounts to a requirement on the asymptotic order of the largest degrees from the ${\bf d}_n$'s. It is known that, in real data, small groups of nodes known as ``hubs"  often have much larger degrees than the rest of the population \cite{mislove2007measurement}, \cite{ahn2007analysis}, \cite{ebel2002scale}, \cite{bryan1999hub}, \cite{csanyi04}, \cite{barabasi99}. The moment condition places a restriction on the how quickly the degrees of hub nodes can grow with resepct to the average degree $\lambda_n$.
%As the final element of the theorem's setting, we fix a sequence of positive integers $\{b_n\}_{n\geq1}$ that correspond to the size of the set $B$ in the variable $\hat s(u:B)$ for each $n$.
% CLT Theorem
Finally for a general node set $[n]$ suppose we are given strengths ${\bf s}$, degrees ${\bf d}$, and a variance parameter $\theta>0$. Given a node $u\in[n]$ and a set $B\subseteq[n]$, define
\begin{equation}\label{eq:mean_func}
\mu(u:B) := \underset{v\in B}{\sum}s_{u,v}
\end{equation}
and
\begin{equation}\label{eq:var_func}
\sigma(u:B) := \sqrt{\underset{v\in B}{\sum}\frac{s_{uv}^2}{d_{uv}}\left(1 - d_{uv} + \theta\right)}
\end{equation}
where $d_{uv}$ and $s_{uv}$ are as in \eqref{eq:duv}. It is easy to check that the above functions are, respectively, the mean and standard deviation of $\hat{s}(u:B)$ under the continuous configuration model on the nodes $[n]$ with parameters ${\bf d},{\bf s}$, and $\theta$ and with arbitrary $\mathcal{P}$. The notations $\mu_n(u:B)$ and $\sigma_n(u:B)$ will be as above but drawing ${\bf d}$, ${\bf s}$, and $\theta$ from the parameter sequence $\{({\bf d}_n, {\bf s}_n, \theta_n, \mathcal{P}_n)\}_{n\geq1}$.
% CLT Theorem
\begin{theorem} \label{thm:CLT}
Let $\{({\bf d}_n,{\bf s}_n,\theta_n,\mathcal{P}_n)\}_{n\geq1}$ be a parameter sequence satisfying Assumptions \ref{assumption:power}-\ref{assumption:distribution}. For each $n\geq1$, let $\hat{\mathcal{G}}_n$ be generated by the continuous configuration model with parameters $({\bf d}_n,{\bf s}_n,\theta_n,\mathcal{P}_n)$.  Fix a node sequence $\{u_n\}_{n\geq1}$ and an integer sequence $\{b_n\}_{n\geq1}$ such that for all $n\geq1$, $u_n\in[n]$ and $b_n\leq 1$. Suppose the parameter sequence $\{d_n(u_n)\}_{n\geq1}$ satisfies
\[
\frac{d_n(u_n)b_n}{n}\rightarrow\infty\text{ as }n\rightarrow\infty
\]
Let $B_n\subseteq[n]$ be a node set chosen, independently of $\hat{\Net}_n$, according to the uniform distribution on all sets of size $b_n$. Then the sequence of random variables $\{\hat s(u_n:B_n)\}_{n\geq1}$ satisfies
\begin{equation}\label{eq:CLT}
\frac{\hat{s}(u_n:B_n) - \mu_n(u_n:B_n)}{\sigma_n(u_n:B_n)}\Rightarrow\mathcal{N}(0,1)\;\text{ as }\;n\rightarrow\infty
\end{equation}
\end{theorem}
% End CLT Theorem

The proof is given in the Appendix. The theorem says that the random variables $\hat{s}(u_n:B_n)$ are asymptotically Normal provided that the sets $B_n$ are ``typical" and that $d(u_n)$ and $B_n$ are sufficiently large. Using the theorem we approximate the pvalue in \eqref{eq:pvalue} by
\begin{equation}\label{eq:pvalue_approx}
p(u:B) \approx 1 - \Phi\left\{\dfrac{s(u:B) - \mu(u:B)}{\sigma(u:B)}\right\}
\end{equation}
where $\mu(u:B)$ and $\sigma(u:B)$ are obtained from the observed network $\mathcal{G}$ according to the specification in \ref{Model:properties}, including setting $\theta$ according to the moment estimator in \eqref{Model:var2}.


\subsection{Overall CCME method}\label{Method:extract}
%ABN: This is the first mention of FDR, alpha.  These should be discussed earlier.
As in Section \ref{Method:update}, denote the set update operation by the map $\Salph: \mathbbm{2}^{[n]} \mapsto \mathbbm{2}^{[n]}$. 
Given a graph $\Net$ and FDR $\alpha$, the basic form of CCME is specified as follows.\vskip0.2cm
\noindent\fbox{\parbox{\textwidth}{
\begin{enumerate}
\item Obtain initial sets $\mathcal{B}_0$ as in Section \ref{Method:initialization}
\item {For each $B\in\mathcal{B}_0$: 
\begin{itemize}
\item Iteratively update $S_{\alpha}(B_t,\Net)\rightarrow B_{t+1}$ until $B_t = B_{t+1}$
\item Add $B_{t+1}$ to a list of communities $\mathcal{C}$
\end{itemize}
}
\item Remove sets from $\mathcal{C}$ that are empty or redundant
\end{enumerate}
}}
%--------------------------------------------Removed
\begin{comment}
The update operation is applied iteratively to every initial set in $B_0(u) \in \mathcal{B}_0$ until a fixed
point is reached, that is, the updated set is identical to the previous set; the case of cycles is discussed below.

 This yields a set of resulting communities $\mathcal{C}$ from which empty and redundant sets are removed.

Letting $J(B_1, B_2):= |B_1\cap B_2|/|B_1\cup B_2|$ be the Jaccard similarity index between two sets, the explicit pseudo-code for the CCME method is given in Algorithm \ref{Method:CCME_alg}.

%ABN: Confusing, notation inconsistent.
\begin{algorithm}
\caption{CCME}\label{Method:CCME_alg}
\scriptsize
\begin{algorithmic}[1]
\State Given $\Net = ([n],E,w)$ and FDR $\alpha\in(0,1)$
\State Initialize detected communities $\mathcal{C} = \phi$
\State Determine initial sets $\mathcal{B}_0$
\While{$|\mathcal{B}_0|>0$}
  \State $B_0\gets \mathcal{B}_0[1]$\Comment{any $\mathcal{B}_0$ element}
  \State Initialize $t \gets 0$ and $B_1 \gets S_\alpha(B_0, \Net)$
  \While{$J(B_{t}, B_{t+1}) < 1$}
    \State $t\gets t+1$
    \State $B_{t+1}\gets S_\alpha(B_t, \Net)$
  \EndWhile
  \State $\mathcal{C} \gets \mathcal{C}\cup\{B_t\}$
  \State $\mathcal{B}_0 \gets \mathcal{B}_0\setminus \{B_0\}$
\EndWhile\label{extractwhile}
\State\textbf{return} $\mathcal{C}_{\text{final}} := $ unique and non-empty communities from $\mathcal{C}$
\end{algorithmic}
\end{algorithm}
\end{comment}
\vskip0.2cm
\noindent Procedural steps similar to (b) and (c) above can be found in the community extraction method ESSC for binary networks \citep{wilson14}. 

A number of practical issues require modifications of the basic procedure described in 
the pseudocode above.  We address these issues, and our modifications, below.

\subsubsection{Iteration cycles} 
It is possible for the set-update procedure to enter a cycle 
$\mathcal{J} := \{B_t,\ldots,B_{t+J}\}$ for which $S_{\alpha}(B_{t+J},\Net) = B_t$. 
In this case we proceed as follows.
\begin{enumerate}
\item If $B_{t+i}\cap B_{t+j} = \phi$ for any two indices $i,j\in\{0,\ldots,J\}$, terminate the iterations and do not store a community
\item{Otherwise, define $B_\mathcal{J} = \cup_{j = 0}^J B_{t+j}$:
  \begin{enumerate}[(i)]
  \item if $B_\mathcal{J}$ has been visited previously, terminate the chain with $B_\mathcal{J}$;
  \item otherwise, restart the chain with $B_{\mathcal{J}}$.
  \end{enumerate}
}
\end{enumerate}
\subsubsection{Near-matches} 
As each extraction is performed independently of the others, CCME can detect communities with arbitrary amounts 
of overlap. However, in rare cases two or more communities in $\mathcal{C}$ will differ only by a small set of 
nodes.  As we prefer not to include near-matches in the final set of communities, in the simulations and 
data analyses that follow, we remove communities having more than $90\%$ of their nodes in another community. 
%The overlap threshold is a general parameter of extraction methods that must be set by protocol; in most cases, we find $90\%$ to be reasonable.

\subsubsection{Filtering of and smart progression through $\mathcal{B}_0$}
In practice, performing an extraction for every initial set in $\mathcal{B}_0$ is time-consuming. 
We add two procedures to CCME to reduce the total number of extractions:\\

\noindent {\bf Filtering $\mathcal{B}_0$.} Here we describe a method to filter the initial sets $\mathcal{B}_0$. Recall from Section \ref{Method:initialization} that each node $u$ yields an initial set $B_0(u)$ which (likely) contains many nodes from the community of $u$. However, if $u$ is not in a community, $B_0(u)$ will not overly represent any community, and an extraction from $B_0(u)$ will (likely) not be fruitful. We can measure the inter-connectedness of nodes in general sets $B$ via the statistic
\[s(B:B) := \underset{v\in B}{\sum}s(v:B\setminus\{v\})\]
Consider that by Theorem \ref{thm:CLT}, $\hat{s}(v:B\setminus\{v\})$ is approximately Normal with mean $\mu(v:B\setminus\{v\})$ and variance $\sigma^2(v:B\setminus\{v\})$ (see Section \ref{Method:CLT}). Hence the sum $s(B:B)$ is approximately Normal with some mean $\mu(B:B)$ and variance $\sigma^2(B:B)$, each derivable from the continuous configuration model. After the transformation
\[
z(B:B):=\frac{s(B:B) - \mu(B:B)}{\sigma(B:B)}
\]
we compute the associated Standard Normal upper-tail p-value assessing the statistical significance of the inter-connectedness of $B$. Before the extractions of CCME, we filter $\mathcal{B}_0$ by performing a multiple-testing correction (described in Section \ref{Method:update}) on the p-values generated by $\{z(B_0(u):B_0(u))\}_{u\in[n]}$.

We note that Theorem $\ref{thm:CLT}$ does not give asymptotic Normality of $\hat{z}(B:B)$ itself: only its components. However we suspect there are true asymptotic results (amenable to statistical inference) for node-set variables like $\hat{z}(B:B)$; these are an area for future research.\\

\noindent {\bf Smart skipping.} As we proceed through $\mathcal{B}_0$, we skip sets that were formed from nodes that have already been extracted into some community. In doing so we avoid many re-extractions of the same community.

\subsubsection{Software}
We provide a complete version of CCME implemented in the \textsc{R} statistical software language. The code is available at https://github.com/jpalowitch/ccme.

























